Confluence via strong normalisation in an algebraic \lambda-calculus with rewriting

The linear-algebraic lambda-calculus and the algebraic lambda-calculus are untyped lambda-calculi extended with arbitrary linear combinations of terms. The former presents the axioms of linear algebra in the form of a rewrite system, while the latter uses equalities. When given by rewrites, algebraic lambda-calculi are not confluent unless further restrictions are added. We provide a type system for the linear-algebraic lambda-calculus enforcing strong normalisation, which gives back confluence. The type system allows an abstract interpretation in System F.

==> eptcsdata.tex <==
\providecommand{\firstpage}{16}
\providecommand{\publicationstatus}{Ronchi della Rocca, S., Pimentel, E. (Eds.): 6th Workshop
on\\ Logical and Semantic Frameworks with Applications 2011 (LSFA 2011).\\
EPTCS 81, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.81.2}{10.4204/EPTCS.81.2}}

